hyppo: A Multivariate Hypothesis Testing Python Package

We introduce hyppo, a unified library for performing multivariate hypothesis testing, including independence, two-sample, and k-sample testing. While many multivariate independence tests have R packages available, the interfaces are inconsistent and most are not available in Python. hyppo includes many state of the art multivariate testing procedures. The package is easy-to-use and is flexible enough to enable future extensions. The documentation and all releases are available at https://hyppo.neurodata.io.

==> validity.tex <==
Validity Proof of K-Sample Test by Dcorr:

Let $Z=[X_1^{1}, X_{1}^{2},\ldots, X_{1}^{n_1}, X_2^{1}, \ldots, X_{k}^{n_k}]$, $Y$ be the one-hot encoding. 

To prove dcorr is valid for K-sample test, it suffices to prove when the null is true, $dcorr(Z,Y) \stackrel{D}{=} dcorr(Z^{\pi},Y)$ for any permutation $\pi$. Then when the null holds, the testing power of the permutation test always equals the type 1 error level. 

Under the null, $X_i^{j} \sim F_{X}$ for any $i,j$. Thus $\pi(X_i^{j}) \stackrel{D}{=} X_i^{j} \sim F_{X}$ for any permutation $\pi$ and any $i,j$. As a result, the concatenated data always distributes the same with or without any permutation. Therefore, $Z \stackrel{D}{=} Z^{\pi}$, $dcorr(Z,Y) \stackrel{D}{=} dcorr(Z^{\pi},Y)$, and the type 1 error level is properly controlled when using Dcorr for K-sample test. 
